e-Fair: Aggregation in e-Commerce for Exploiting Economies of Scale

In recent years, many new and interesting models of successful online business have been developed, including competitive models such as auctions, where the product price tends to rise, and group-buying, where users cooperate obtaining a dynamic price that tends to go down. We propose the e-fair as a business model for social commerce, where both sellers and buyers are grouped to maximize benefits. e-Fairs extend the group-buying model aggregating demand and supply for price optimization as well as consolidating shipments and optimize withdrawals for guaranteeing additional savings. e-Fairs work upon multiple dimensions: time to aggregate buyers, their geographical distribution, price/quantity curves provided by sellers, and location of withdrawal points. We provide an analytical model for time and spatial optimization and simulate realistic scenarios using both real purchase data from an Italian marketplace and simulated ones. Experimental results demonstrate the potentials offered by e-fairs and show benefits for all the involved actors.

==> constraint-table.tex <==
\begin{table*}[!t]
	\centering
	\caption{Constraints applied to the optimization model distinguished by second and third phases (upper and lower parts).}
	\label{tab:constraints}
	\begin{tabular}{r|c|l}
		\toprule
		Constraint expression & scope & Description \\
		\midrule
		\(\displaystyle \sum_{i=1}^{I} x_{i} =  y_{fair} 		\) & $\forall Fair$ 
		& The number of purchased products is equal to the number of products requested in the fair.\\
		\(\displaystyle \sum_{l=1}^{L} \delta_{i}^{(l)}  = x_i \)  & $\forall S_i$ 
		%& The sum of all interval selection variables is equal to the quantity of sold products by seller $S_i$. \\
		& The sum of variables of all the $L$ intervals is equal to the quantity of sold products by seller $S_i$. \\
		\(\displaystyle x_{i} \leq e_{i} 		\) & $\forall i$ 
		& The number of products sold  by seller $S_i$ is less than or equal his supply available.\\ \newline
		
		\(\displaystyle \Delta^{(l)}_{i} w_{i}^{(l)} \leq \delta^{(l)}_{i} \leq \Delta^{(l)}_{i} w_{i}^{(l-1)} \) & $\forall i,l$ 
		& Set of L inequalities which define the bounds of the $\delta_{i}^{(l)}$ quantities throw binary control variables $w_i$.\\
		\midrule
		\(\displaystyle \sum_{j=1}^{J} x_{ij} = x_{i}     \) & $\forall i$ 
		& The sum of shipped products in each trajectory is equal to the quantity of sold products by the seller $S_i$.\\
	
		\(\displaystyle x_{ij} 	\leq a_{ij} \cdot y_{fair}  \) & $\forall i,j$ 
		& When the arc $i \rightarrow j$ is used (i.e. $x_{ij} > 0$), the amount of products to be shipped from \emph{i}-th seller can be \\ & & 
		no larger than the total fair demand, which is always true. Consequently, shipment cost $S$ can be applied \\ & & only if the arc is used, because necessarily $a_{ij} = 1$.\\ %a) Shipping cost S along the arc $i \rightarrow j$ applies only if the arc is effectively used, i.e. $x_{ij} > 0$.
		\(\displaystyle \sum_{i=1}^{I} x_{ij} \leq c_{j} 	\) & $\forall j$ 
		& The sum of products shipped to a POP is less than or equal to the POP capacity. \\
		\(\displaystyle \sum_{j=1}^{J} y_{jk} = y_{k}     	\) & $\forall k$ 
		& The quantity of products requested by the buyer is divided among POPs. \\
		\(\displaystyle \sum_{j=1}^{J} b_{jk} 	= 1  		\) &$ \forall k$ 
		& The buyer withdraws his products by only one POP.\\
		\(\displaystyle \sum_{i=1}^{I} x_{ij} 	= \sum_{k=1}^{K} y_{jk}  \)  & $\forall j $ 
		& The amount of incoming products at POP is equal to the amount of outgoing products (flow equation).\\
		
		\(\displaystyle \Gamma^{(m)} u^{(m)}\leq \gamma^{(m)} \leq \Gamma^{(m)} u^{(m-1)} \) & $ \forall m $
		& Set of M inequalities which define the bounds of the $\gamma^{(l)}$ quantities throw binary control variables $u$.\\
					\(\displaystyle y_{jk} \leq b_{jk} \cdot y_{fair}  \) & $\forall j,k$ 
		& When the arc $j \rightarrow k$ is used (i.e. $y_{jk} > 0$), the amount of products to be retrieved from \emph{k}-th buyer is no \\ & & larger than the total fair demand, which is always true. Consequently, pick up cost $d_{jk}$ can be applied \\ & & only if the arc is used, because necessarily $b_{jk} = 1$.\\ %a) Distance-related costs along the arc $j \rightarrow k$ applies only if the arc is effectively used, i.e. $y_{jk} > 0$. \\ 
		% the second is the total number of withdrawals to POPs
		\(\displaystyle \sum_{m=1}^M \gamma^{(m)} = \sum_{j=1}^J\sum_{k=1}^{K} b_{jk}  \) & $\forall j$ 
		%& The sum of all interval selection variables for the considered POP provider is equal to the total number of withdrawals \\& 
		%& to POPs. \\
		& The sum of variables of all the $M$ intervals for the considered POP provider is equal to the total number \\ & & of withdrawals to POPs. \\
		\(\displaystyle x_{ij} \geq 0 						\) & $\forall i,j$ 
		& The quantity of products along each arc $i \rightarrow j$ is non-negative. \\
		\(\displaystyle y_{jk} \geq 0 						\) & $\forall j,k$ 
		& The quantity of products along each arc $j \rightarrow k$ is non-negative.\\
		\bottomrule
	\end{tabular}
\end{table*}

